PALLM: Evaluating and Enhancing PALLiative Care Conversations with Large Language Models

Effective patient-provider communication is crucial in clinical care, directly impacting patient outcomes and quality of life. Traditional evaluation methods, such as human ratings, patient feedback, and provider self-assessments, are often limited by high costs and scalability issues. Although existing natural language processing (NLP) techniques show promise, they struggle with the nuances of clinical communication and require sensitive clinical data for training, reducing their effectiveness in real-world applications. Emerging large language models (LLMs) offer a new approach to assessing complex communication metrics, with the potential to advance the field through integration into passive sensing and just-in-time intervention systems. This study explores LLMs as evaluators of palliative care communication quality, leveraging their linguistic, in-context learning, and reasoning capabilities. Specifically, using simulated scripts crafted and labeled by healthcare professionals, we test proprietary models (e.g., GPT-4) and fine-tune open-source LLMs (e.g., LLaMA2) with a synthetic dataset generated by GPT-4 to evaluate clinical conversations, to identify key metrics such as `understanding' and `empathy'. Our findings demonstrated LLMs' superior performance in evaluating clinical communication, providing actionable feedback with reasoning, and demonstrating the feasibility and practical viability of developing in-house LLMs. This research highlights LLMs' potential to enhance patient-provider interactions and lays the groundwork for downstream steps in developing LLM-empowered clinical health systems.

==> figures-and-tables/summary-table.tex <==

% \begin{table}[]
% \caption{Summary of the 'Best Practice' principles of quality patient-provider communication which guide the design of CommSense, outlining metrics and citations, identification tags, operationalization ideas, engineering tools for implementation, and rules for identification (Adapted from \cite{lebaron2023commsense}). Taking ``UNDERSTANDING'' as an example, we will examine whether the clinicians do a ``good'' job in exploring/seeking understanding by evaluating whether they use open-ended questions with end-to-end open-ended question detection models. Detected open-ended questions in each segment of the conversation will indicate a ``Good Understanding'' segment.}
% \label{tab:summarization-commsense}
% \scriptsize
% % \footnotesize
% \begin{tabularx}{1\textwidth}{
%   >{\hsize=0.55\hsize}X
%   >{\hsize=0.85\hsize}X
%   >{\hsize=1\hsize}X
%   >{\hsize=1.3\hsize}X
%   >{\hsize=1.3\hsize}X
%   }
% \hline
% \textbf{Metric and Citations} & \textbf{Ground Truth to Identify} & \textbf{Ideas of How to Operationalize} & \textbf{Computational Tools for Automation} & \textbf{Computational Implementation Rules} \\ \hline
% Explore/ seek understanding \cite{wittenberg2018comfort,wittenberg2018communicating,geerse2019qualitative,ferrell2020enhancing} & 
% UNDERSTANDING (good) & 
% Use of open-ended questions/ statements. & 
% End-to-end open-ended question detection \cite{wan2016modeling}. \newline \gray{(training machine learning models based on Amazon Question and Answer Dataset \cite{AmazonQA})} & 
% {[}Good Understanding{]} \newline Detected open-ended question statements 
% \\ \hline
% Convey empathy/ compassion \cite{long2011ten,long2011ten,boyle2017palliative,moore2018communication,jain2020goals,pajka2021feasibility,schwartz2021physician} & 
% EMPATHY (good) \newline \gray{Name; Understand; Respect; Support} & 
% Use of specific phrases/ words & 
% End-to-end empathy seeking/ providing detection \cite{hosseini2021takes}. \newline \gray{(training machine learning models to identify statements seeking empathy vs. providing empathy vs. neutral with public dataset \cite{MahhosEmpathy}.)} & 
% {[}Good Empathy{]} \newline Detected empathy providing statements 
% \\ \hline
% Elicit emotion; Allow to express emotion; Respond to emotion \cite{back2007efficacy,kwok2020evaluation,pajka2021feasibility,jain2020goals,back2020patient,wittenberg2018communicating,sommovilla2019discussing} & 
% EMOTION (good) \newline \gray{Respond/Allow};  \newline \newline EMOTION (bad) \newline \gray{Dismiss/ Deflect/ Intellectualize} & 
% $\circ$ Ignore/ deflect/ dismiss/ change subject; \newline $\circ$  Respond to emotion with cognitive facts/ figures; \newline $\circ$ Pause for 10 seconds after delivering difficult news (allow space/ time for patient to process emotion) & 
% $\circ$ Detection of \newline 1) concordance of emotional tone; \newline 2) response to emotion with cognitive statements; \newline using Linguistic Inquiry Word Count (LIWC) analysis \cite{tausczik2010psychological}: \newline \gray{level of emotion; level of cognitive process; emotional tone (positive/ negative);} \newline $\circ$ Detection of proper pause via acoustic analysis and silence detection & 
% {[}Good Emotion{]} \newline 1. the clinician's emotion direction (pos vs. neg) is cohered with the patient's \newline 2. Pause 10 seconds after statement with negative emotion and sadness; \newline {[}Bad Emotion{]} \newline 1. Response patient's high emotion level statement with high cognitive process level statement; \newline 2. Miss to pause after detected statement with highly negative emotion and sadness 
% \\ \hline
% Be present \cite{long2011ten,bernacki2014communication,wittenberg2018communicating,moore2018communication,sommovilla2019discussing,geerse2019qualitative,paladino2020patient} & 
% SILENCE (good) \newline ACTIVE LISTENING (good); \newline \newline SILENCE (bad) \newline INTERRUPTION (bad) & 
% $\circ$  Allow silence / pauses <50\% talking; \newline $\circ$ Active listening [Reflect back/ confirm understanding/ restate essential information/ paraphrase]; \newline $\circ$ Avoid interruptions/ talking over & 
% $\circ$ Detection of talking ratio, pause, and interruptions via acoustic analysis: \newline 
% \gray{voice identification; silence detection; overlap detection} \newline $\circ$ Identification of paraphrase based on semantic similarity \cite{yin2015convolutional} & 
% {[}Good Present{]} \newline 1. (Overall) Allow silence throughout the conversation; \newline 2. (Overall) < 50\% talking; \newline 3. Detected paraphrase indicated by semantic similarity value; \newline {[}Bad Present{]} \newline Detected interruptions 
% \\ \hline
% Be clear \cite{baile2005patient,long2011ten,mazor2013patients,gilligan2018patient,wittenberg2018communicating,martin2019communication,paladino2020patient,back2020patient} & 
% LANGUAGE (good) \newline \gray{Explained/ Clear}; \newline \newline LANGUAGE (bad) \newline \gray{Unexplained/ Unclear} & 
% $\circ$ Use plain, direct language [active voice, use second person, sentences <15 words]; \newline $\circ$  No/ limited medical jargon; \newline $\circ$  Contextualize/ indicate next step & 
% $\circ$ Detection of plain language using LIWC analysis: \newline \gray{word and sentence count; words per sentence; level of cognitive process; first and second pronouns} \newline $\circ$ Detection of medical jargon based on medical dictionary \cite{HarvardMedicalDictionary} & 
% {[}Good Clarity{]} \newline 1. (Overall) Use more second pronouns and less first pronouns than usual value; \newline 2. (Overall) Statements are with low level of cognitive process in average; \newline {[}Bad Clarity{]} \newline 1. Detected overuse of medical jargon; \newline 2. Word per sentence > 15 
% \\ \hline
% \end{tabularx}
% \end{table}

\begin{table}[]
\caption{Summary of the guiding 'Best Practice' principles for quality patient-provider communication in the design of CommSense, outlining metrics with citations, identifiers, operationalization concepts, implementation tools, and rules (adapted from \cite{lebaron2023commsense}). For instance, we evaluate the clinician's ability to explore/seek understanding (tagged as "UNDERSTANDING") by detecting the usage of open-ended questions using an end-to-end model. A segment containing detected open-ended questions is classified as exhibiting "Good Understanding".}
\label{tab:summarization-commsense}
\scriptsize
% \footnotesize
\begin{tabularx}{1\textwidth}{
  >{\hsize=0.55\hsize}X
  >{\hsize=0.85\hsize}X
  >{\hsize=1\hsize}X
  >{\hsize=1.3\hsize}X
  >{\hsize=1.3\hsize}X
  }
\hline
\textbf{Metric} & \textbf{Grount Truth Tags} & \textbf{Operationalization Concepts} & \textbf{Computational Tools for Implementation} & \textbf{Rules for Computational Implementation} \\ \hline
Understanding \cite{wittenberg2018comfort,wittenberg2018communicating,geerse2019qualitative,ferrell2020enhancing} & 
UNDERSTANDING (good) & 
Employment of open-ended questions/ statements. & 
End-to-end open-ended question detection \cite{wan2016modeling}. \newline \gray{(Training machine learning models on Amazon Question and Answer Dataset \cite{AmazonQA})} & 
{[}Good Understanding{]} \newline Open-ended question statements detected
\\ \hline
Empathy \cite{long2011ten,long2011ten,boyle2017palliative,moore2018communication,jain2020goals,pajka2021feasibility,schwartz2021physician} & 
EMPATHY (good) \newline \gray{Name; Understand; Respect; Support} & 
Utilization of specific phrases/ words & 
End-to-end empathy seeking/ providing detection \cite{hosseini2021takes}. \newline \gray{(Training machine learning models to categorize statements as empathy seeking, empathy providing, or neutral using a public dataset \cite{MahhosEmpathy})} & 
{[}Good Empathy{]} \newline Empathy-providing statements detected 
\\ \hline
Emotion \cite{back2007efficacy,kwok2020evaluation,pajka2021feasibility,jain2020goals,back2020patient,wittenberg2018communicating,sommovilla2019discussing} & 
EMOTION (good) \newline \gray{Respond/Allow};  \newline \newline EMOTION (bad) \newline \gray{Dismiss/ Deflect/ Intellectualize} & 
$\circ$ Avoid deflecting/ dismissing/ changing the subject; \newline $\circ$  Respond to emotion with factual information; \newline $\circ$ Pause for 10 seconds following the delivery of difficult news (allowing time for patient emotional processing) & 
$\circ$ Detection of \newline 1) emotional tone concordance; \newline 2) cognitive response to emotional statements; \newline using Linguistic Inquiry Word Count (LIWC) analysis \cite{tausczik2010psychological}: \newline \gray{emotion level; cognitive process level; emotional tone (positive/ negative);} \newline $\circ$ Silence detection and acoustic analysis for proper pause detection & 
{[}Good Emotion{]} \newline 1. Clinician's emotion direction (positive vs. negative) aligns with the patient's \newline 2. 10-second pause after a statement with negative emotion; \newline {[}Bad Emotion{]} \newline 1. Respond to high emotion level statement with high cognitive process level statement; \newline 2. No pause after a statement with highly negative emotion 
\\ \hline
Presence \cite{long2011ten,bernacki2014communication,wittenberg2018communicating,moore2018communication,sommovilla2019discussing,geerse2019qualitative,paladino2020patient} & 
SILENCE (good) \newline ACTIVE LISTENING (good); \newline \newline SILENCE (bad) \newline INTERRUPTION (bad) & 
$\circ$  Encourage silence / pauses <50\% of the conversation; \newline $\circ$ Active listening [Reflection/ confirmation of understanding/ essential information restatement/ paraphrasing]; \newline $\circ$ Avoid interruptions/ talking over & 
$\circ$ Detection of speech ratio, pauses, and interruptions via acoustic analysis: \newline 
\gray{voice identification; silence detection; overlap detection} \newline $\circ$ Paraphrase identification based on semantic similarity \cite{yin2015convolutional} & 
{[}Good Presence{]} \newline 1. (Overall) Encourage silence; \newline 2. (Overall) Engage in conversation < 50\% of the time; \newline 3. Detected paraphrasing indicated by semantic similarity score; \newline {[}Bad Presence{]} \newline Interruptions detected
\\ \hline
Clarity \cite{baile2005patient,long2011ten,mazor2013patients,gilligan2018patient,wittenberg2018communicating,martin2019communication,paladino2020patient,back2020patient} & 
LANGUAGE (good) \newline \gray{Explained/ Clear}; \newline \newline LANGUAGE (bad) \newline \gray{Unexplained/ Unclear} & 
$\circ$ Utilize plain, direct language [active voice, use second person, sentences <15 words]; \newline $\circ$  Limit medical jargon; \newline $\circ$  Contextualize/ indicate next steps & 
$\circ$ Detection of plain language using LIWC analysis: \newline \gray{word and sentence count; words per sentence; cognitive process level; usage of first and second pronouns} \newline $\circ$ Detection of medical jargon based on medical dictionary \cite{HarvardMedicalDictionary} & 
{[}Good Clarity{]} \newline 1. (Overall) Use more second pronouns and less first pronouns than usual; \newline 2. Using medical jargon with explanation provided; \newline {[}Bad Clarity{]} \newline 1. Detected overuse of medical jargon; \newline 2. Long sentences (words per sentence > 15)
\\ \hline
\end{tabularx}
\end{table}

